Maximizing science return by coordinating the survey strategies of Roman with Rubin, and other major facilities

[Abridged] The Nancy Grace Roman Space Telescope will be one of several flagship survey facilities operating over the next decade starting $\sim$2025. The deep near-IR imaging that Roman will deliver will be highly complementary to the capabilities of other survey telescopes that will operate contemporaneously, particularly those that can provide data at different wavelengths and messengers, or different time intervals. Combining data from multiple facilities can provide important astrophysical insights, provided the data acquisition is carefully scheduled, and careful plans are made for appropriate joint data analyses. In this White Paper, we discuss the broad range of science that would be enabled by coordinating Roman observations of the Galactic Bulge with those of the Vera C. Rubin Observatory. Specifically, we discuss how Roman's characterization of lensing events caused by exoplanets, stellar systems and stellar remnants can be enhanced by data from Rubin. The same data will also be highly advantageous for the determination of stellar properties, and for distinguishing exoplanetary transits. It will enable more accurate period-color-luminosity relationships to be measured for RR~Lyrae throughout the Milky Way Bulge and Bar, probing galactic structure and dynamics. But we stress that this is only a sample of the full potential and advocate for a more complete study to be made as a joint effort between these major projects. We note that we do not suggest any changes beyond the established Science Requirements for the RGBTDS, in terms of survey footprint or filter selection.

==> notes.tex <==
Useful links and possible papers to consider/cite

% https://www.stsci.edu/files/live/sites/www/files/home/roman/_documents/roman-capabilities-stars.pdf

% The Definitive Map of the Galactic bulge https://arxiv.org/pdf/1812.08670.pdf

% Simulating the Legacy Survey of Space and Time stellar content with TRILEGAL - https://arxiv.org/pdf/2208.00829.pdf

% The Mira-based Distance to the Galactic Center https://iopscience.iop.org/article/10.3847/1538-4357/aad7fb/pdf

% https://arxiv.org/pdf/1812.04445.pdf

Science Pitch Proposals for Roman:

Daisuke KawataMSSL, UCL, UK

Naoteru Gouda (NAOJ), Takafumi Kamizuka (The University of Tokyo), Hajime Kawahara (ISAS/JAXA), Naoki Koshimoto (NASA Goddard/UMD), Shota Miyazaki (ISAS/JAXA), Shogo Nishiyama (Miyagi University of Education), Ryou Ohsawa (NAOJ), Daisuke Suzuki (Osaka), Masahiro Takada (Kavli IPMU/Tokyo)

Roman+JASMINE Galactic Center Astrometry Survey

The Galactic center region (Rgc<~100 pc), including the Nuclear Star Cluster and Nuclear Stellar Disk, is the heart of our Galaxy and the place holding the historical treasures accumulated since the beginning of the formation of the Galaxy. It is also the highest density region of the Galaxy, harbouring the super massive black hole (SMBH). In the last decades, multi-wavelength observations have revealed fascinating phenomena, such as the motion of the stars around SMBH, the Fermi bubble, various high-energy sources, intermediate mass BH candidates and the complex structure of the central molecular zone. However, because of the severe dust extinction and the large and dense stellar structure, the measurements of stellar kinematics in the Galactic center are still limited, due to the small field of view (FoV) of high-resolution space or adaptive optics (AO) near-infrared (NIR) facilities and the limited spatial resolution of the large FoV facilities. With its unique survey capability with wide-field, high-resolution and high-sensitivity, the Nancy Grace Roman Space Telescope is the ideal facility to explore the Galactic center stellar structure and also 5 years of operation enables the measurements of the proper motion of the stars, i.e. astrometry. The precise astrometry will open up the new sciences, such as detecting long-time-scale (>100 days) astrometric microlensing event due to the black holes (e.g. Toki & Takada arXiv:2103.13015; Sajadian & Sahu arXiv:1301.03812), measuring the age distribution of the kinematically selected nuclear stellar disk, which will tell us the formation epoch of the Galactic bar (e.g. Baba & Kawata 2020, MNRAS, 492, 4500) and testing the existence of the Ultra Light Dark Matter (10^-22 - 10^-18 eV) core (e.g. Toguz et al. 2022, MNRAS, 511, 1757).<br><br>Hence, we propose to observe the Galactic center field of |l|<0.5 deg and |b|<0.4 deg (~5 pointings) with three filters at least twice per year when the Galactic center is observable. This field overlaps with the Galactic Center Survey field of the Japanese NIR astrometry mission, JASMINE, planned launch in 2028 by ISAS/JAXA. Taking an advantages of the similar operation period of Roman to JASMINE, we propose to observe this field with 5 sets of dithering observations (~20 images per filter to sample PSF) with 3 different filters, taking the shallow images with F087 (not saturate for 15 mag stars, but also deep enough to ensure the astrometric accuracy of faint stars) and the deep images with F158 (<~21 mag) and F213 (<~21 mag). Note that the final choices of the size of the field, filters and the depth are subject to further studies. The shallow images with F087 can avoid the saturation of the astrometric reference bright stars whose astrometry is accurately measured by JASMINE (J<12.5 mag) and Gaia (G<16 mag), which will be used to calibrate astrometry of the fainter stars (F087~20 mag). The calibrated astrometry for the fainter stars in F087 images will be used for the reference stars for the deeper images with F158 and F213. We aim to reach the well calibrated proper motion of ~0.03 mas/yr (~1.2 km/s velocity uncertainty at the distance to the Galactic center) for a few million stars of <21 mag stars in F158 (c.f. WFIRST Astrometry Working Group 2018, JATIS, 5, 044005; Hosek et al. 2022, ApJ, 939, 68). F213 images will be used to measure the colour of the faint stars and also detect the fainter sources, including the microlensing event. The proposed field will be also observed by Subaru's next generation AO instrument, ULTIMATE-SUBARU. Hence, the legacy value of the Roman+JASMINE Galactic Center Survey will be extremely high. Combination with ULTIMATE-SUBARU observations of additional few years will increase the potential to find long time-scale phenomena, such as the astrometric microlensing by the intermediate mass BH (100-100,000 Msun), which would be a revolutionary discovery, even if one event is detected. The data will be also valuable for the geometric distortion calibration for the other Roman observations. Our team is developing the astrometric analysis tools for JASMINE and ULTIMATE-SUBARU, and we wish to work with the other astrometry experts in the Roman community to maximise the synergies of these upcoming novel and unique NIR facilities.

Galactic Bulge Time Domain Survey

stellar populations and the interstellar medium: Stellar Populations: Astrometry Stellar Populations: Galactic center, Stellar Populations: Galaxy evolution, Stellar Populations: Gravitational microlensing, Stellar Populations: Star clusters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Daisuke Suzuki
Osaka Univeristy

Naoki Koshimoto(NASA Goddard/UMD), Shota Miyazki(ISAS/JAXA), Takahiro Sumi(Osaka U)

Black Hole Microlensing Survey with Roman and ULTIMATE-Subaru toward the Galactic Center

We propose to observe the Galactic center region (|l|<0.5 deg and |b|<0.4 deg) by using F213 filter with a cadence of at least every 5 days (TBD, higher the cadence is the better) to find and characterize the black hole (BH) microlensing events. Although some BH microlensing events are expected to be found by the Roman Galactic Exoplanet Survey in their nominal survey bulge field that are not including the Galactic center, the proposed observational field includes the nuclear stellar disk whose population could be different from those of the bulge. We will use both photometric and astrometric information for the light curve and astrometric microlensing signals to find/characterize the BH microlensing events.<br><br>This can be done only by the instruments with wide FOV, high angular resolution and K-band filter, because this area is a relatively large, very dense, and highly obscured region by the interstellar dust.<br><br>This field will be observed by the ground-based NIR PRIME telescope and Japanese NIR astrometry mission, JASMINE. But, PRIME is seeing-limited and uses H-band, and JASMINE can detect only bright stars for the very precise astrometry measurement. ULTIMATE-Subaru will also monitor the Galactic center with GLAO (14' x14' FOV and ~0.4" seeing) and K-band to find the BH microlensing events, which will be a powerful survey program if realized, but the Galactic center is only visible in summer from Hawaii. By combining the Roman data, these survey data become highly valuable, because the light curve coverage is complementary to each other to measure the satellite and orbital parallax signals and to constrain the astrometric microlensing signals. ULTIMATE-Subaru will be online in late 2020s, but precursor Roman observation will be important especially to measure the astrometric microlensing signals.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Gravitational microlensing,

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
	
Jan Skowron
Astronomical Observatory, University of Warsaw
		
More consistent color measurements of the microlensing source stars

During the Galactic Bulge Time Domain Survey it is planned to continuously monitor microlensing events in a single wide band (F146) to measure the basic light curve parameters. It is stated that the 7 fields will be monitored in a bluest filter for one exposure every 12 hours in order to measure the color of the microlensing source stars. The bluest filter is F062. While this strategy is sufficient to measure colors of G and K stars, it might be problematic for the large number of microlensing sources, i.e. M-dwarf stars. In order to facilitate even better measurements of masses of the discovered exoplanets, I propose a slight change in this strategy.<br><br>The spectral energy distribution of M dwarfs peaks within the F146 wide filter and falls rapidly toward shorter wavelengths. Additionally, significant extinction is present in the monitored fields further diminishing any signal in the F062 filter. Most of the M-dwarf source stars will be blended with the M-dwarf lenses. All these factors yield very low signal-to-noise measurements of the colors of source stars. A much better choice for the M-dwarf would be a F087 filter, however, the separation between its wavelength and the wide-band filter is not sufficient, leading to weak leverage for the measurement for all stars. I propose to add occasional exposures in one of the red filters of standard width, for example F158, as well as F087. A pair of F087 and F158 measurements would yield high signal-to-noise color measurement for M-dwarfs. The measurements in F062 will allow for better characterization of hotter stars. The sub-1-day cadence in one of the filters is preferable in order to get the color information for the shortest events, however is not necessary in all filters. The additional color information (in one red and another blue filter) gathered every 1-3 days would benefit the great majority of events and will not interfere with the main survey goals. Such additional, continuous color data will also benefit other astrophysical studies in the time domain.

Galactic Bulge Time Domain Survey

exoplanets and exoplanet formation, stellar physics and stellar types, Exoplanets, Exoplanet detection methods, Free floating planets, Variable stars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	
	
Kishalay De
Massachusetts Institute of Technology

Revealing the obscured and dynamic Galactic bulge with a wide area survey

Stellar variability forms one of the corner stones of modern astronomy. From stellar pulsations in the smallest white dwarfs to ellipsoidal variability in the largest giants, optical time domain surveys combined with the unprecedented astrometric capabilities of missions like Gaia are revolutionizing our understanding of stellar life cycles and populations -- essentially re-writing textbooks underpinning every area of astrophysics. Yet current optical datasets remain severely limited in terms of understanding Galactic scale demographics of variability, as well as finding rare stages in stellar evolution due to the extremely small accessible volume in the dust obscured Galactic plane. Only in the last few years have shallow infrared time domain surveys from the ground begun to unravel this hidden landscape of variability, with infrared time domain datasets expected to grow exponentially by the time of start of the Roman mission.<br><br>The Roman space telescope's Galactic bulge time domain survey is poised to be a game changer in our understanding of exoplanet demographics via microlensing searches. Yet, the exceptional infrared sensitivity and spatial resolution of the same surveys can revolutionize the field of stellar astronomy with minor modifications to the survey design aimed at increasing the effective stellar mass footprint. As the exact footprint of the Roman Galactic Exoplanet Survey remains to be confirmed, we recommend that the survey covers a large footprint than the planned 2.0 sq. deg. patch in the Galactic bulge (Penny et al. 2019). This could be achieved, for instance, by lowering the average cadence in the footprint, or by selecting a wider patch (~ 10 sq. deg.) meant for lower cadence monitoring (~ 1 day). We stress that even lower cadence data on this extremely rich (but yet optically inaccessible due to dust obscuration) stellar fields near the Galactic center will provide a golden dataset for stellar astronomy, revealing clues to historic unanswered questions ranging from the population of low frequency gravitational wave sources like close binary white dwarfs (e.g. Burdge et al. 2019), close binaries on their approach to merger (e.g. Tylenda et al. 2011) to hidden black holes lurking around luminous companions (e.g. El. Barry et al. 2022). This dataset will be ideally placed to capitalize on synergies with ongoing and near-future shallower surveys in the infrared (e.g. PRIME, WINTER, DREAMS, Gattini-IR) as well as the upcoming Vera Rubin Observatory.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Binary stars, evolved stars, variable stars, neutron stars, stellar evolution

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
László Molnár
Konkoly Observatory, CSFK, Budapest

Csilla Kalup, Rozália Ádám, Róbert Szabó

Deep survey and asteroseismology of obscured Galactic globular clusters

The bulge is home to many globular clusters. A number of them are far away or obscured by dust. Some of these have been discovered only recently, and a few of them have never been studied in detail, although they are expected to contain various types of variable stars, just like their brighter counterparts. However, as results from ground-based and space-based time series photometry show, variable stars such as the RR Lyrae population of the cluster, blue stragglers, eclipsing binaries, and oscillating red giants provide a wealth of information about the cluster. These include photometric metallicities (of the RR Lyrae stars), constraints on the formation of eclipsing binaries, mass loss histories, or distance estimates.<br><br>In particular, the Kepler space telescope has shown that longitudinal observations of globular clusters can be very valuable. Seismic parameters could be derived for giants in the cluster M4, which was also the target of an extensive variability search. Upcoming work on other K2 clusters (M80, NGC 5897) will show how precise photometry of cluster RR Lyrae stars can be used to obtain detailed pulsation profiles and signatures for these stars, allowing us to estimate their physical parameters. Roman could achieve similar success but its more powerful optics and infrared filter would make it possible to target the obscured and/or distant clusters around the bulge, too. Furthermore, multicolor photometry, especially at the turn-off point, the main sequence, and the normal and extreme horizontal branches, can be used to unravel the star formation history of a cluster. Placing the fields of the Bulge survey, either in the nominal mission or during an extension, in such a way that they encompass one or more clusters will give us a truly unique opportunity to study globular clusters in these ways.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Globular star clusters, Variable stars, Star formation, Population II stars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

László Molnár
Konkoly Observatory, CSFK, Budapest

Róbert Szabó

Asteroseismology of lensed stars in the bulge

Microlensing events magnify the stellar source by 10 to 1000 times its normal brightness, briefly bringing it within the range of instruments that would otherwise not be sensitive enough to detect it. This can be exploited in a variety of ways, such as recording the spectra of magnified dwarf stars within the Galactic Bulge. Photometric observations, on the other hand, allow us to detect the variability of the source if the lensing event is slow enough. Einstein timescales of Bulge microlensing events range from a few days to about a hundred days, with an average of 22 days. Longer events thus have the ability to significantly magnify the source for a few weeks. This is comparable to a 27-d observation in a single TESS sector, and single-sector data have been used to determine seismic parameters of stars in that mission.<br><br>Many parameters will determine whether Roman is able to extract seismic information for a lensing source. However, given enough amplification, the 15-minute cadence of the Bulge survey and the limited amount of time a source is sufficiently magnified can give us an idea of what sources to expect. Stars with lower oscillation frequencies will have higher amplitudes, but short observations will be limited to frequencies of maximum amplitude (nu_max) above a few to 10 microHz. The cadence gives us an upper limit of a few hundred microHz, but at high values the mode amplitudes are also much lower and may not be detectable at all. Based on the TESS single-sector observations analyzed by Stello et al. (2022), red clump stars are best suited for observations: they are sufficiently bright and their oscillations are in the right range with nu_max values around 30-40 microHz. Further simulations would certainly be needed to calculate a realistic yield for Roman observations: however, any seismic detection of a Bulge star would be a significant achievement for the Roman space telescope.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, Variable stars, Evolved stars, Gravitational microlensing

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
László Molnár
Konkoly Observatory, CSFK, Budapest

Susmita Das

Precision photometry and seismology of pulsating stars across the Milky Way

Classical pulsating stars are extremely important distance estimators because of their well-defined period-luminosity (PL) relations. However, at present, one of the primary hindrances in the precise calibration of the PL relations arises from the inability to accurately determine the effect of metallicity on the PL relations. RR Lyrae stars offer us the advantage of estimating their metallicities from their light curve structures, which in turn requires precise photometric data.<br><br>To this end, the simultaneous and precise photometry and spectroscopy of RR Lyrae stars in the Milky Way from the Nancy Grace Roman Space Telescope would prove crucial in the comparison of the photometric and spectroscopic metallicities of the particular stars. Photometric metallicity estimates can be calibrated from known or measured spectroscopic values, and then estimates can be given for stars that are too faint for spectroscopy, well within obscured regions or at large distances. The derived period, brightness and metallicity values can then be used for a precise calibration of the period-luminosity-metallicity (PLZ) relation.<br><br>Furthermore, precise, high-cadence photometry of classical pulsating stars can reveal a multitude of low-amplitude modes, providing us with detailed seismic signatures. Some of these modes are understood well enough to be modeled, and can be used to infer physical properties for classical pulsating stars. Continuous light curves from Roman will make it possible to determine the intrinsic variability of these modes and to compare them to the long-term observations of the OGLE survey. Roman will also allow us to survey seismic signatures of pulsating stars deep within the bulge and on the far side of the Milky Way, far outside the reach of the Kepler and TESS space telescopes.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Variable Stars, Stellar abundances,

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Marc Pinsonneault
Professor of Astronomy, the Ohio State University

Tim Bedding (U Sydney), Scott Gaudi (OSU), Marc Hon (U Hawaii), Daniel Huber (U Hawaii), Matthew Penny (LSU), Sanjib Sharma (Johns Hopkins), and Dennis Stello (UNSW)

Asteroseismology in the Galactic Bulge

Red giants oscillate, and these oscillations can be used as powerful diagnostics of global stellar properties. Time domain surveys from space - CoRoT, Kepler, K2 and TESS - have been able to characterize these asteroseismic properties in large samples of stars. However, other missions are limited to relatively nearby, bright targets (because of small apertures) or uncrowded fields (due to large pixels). The Roman Galactic Bulge Time Domain Survey is well-suited for asteroseismology of the crucial, and poorly understood, stellar populations in the center of the Galaxy. Oscillations will have lower amplitude in the IR than the visible, but they should still be detectable. The high spatial resolution of Roman, its relatively large aperture, and the ability to see deep into the Galactic center at infrared wavelengths all make Roman a potent engine for studying stellar populations that are not accessible with other time domain surveys. Ultra-precise astrometry will give powerful independent constraints on asteroseismic masses and radii, and complementary information from stellar granulation may also be obtainable. The notional cadence, area, and dwell of the Galactic Bulge Time Domain Survey are reasonably well-matched to those required for asteroseismology. However, some modification of these and other survey parameters may enable additional transformative stellar science.<br><br>Masses from asteroseismology can allow us to measure the distribution of ages; when combined with spectroscopic and astrometric surveys, we can also reconstruct the chemical and kinetic evolution of our bulge, permitting a much more complete picture of the formation and evolution of the Milky Way Galaxy. This program will therefore have synergy with other survey science, such as interpreting transit and microlensing demographics or stellar remnant mass functions.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Galaxy bulges, Late-type stars, Stellar evolution, Stellar abundances, Variable stars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Matthew Digman
Montana State University

Chris Hirata

Multi-messenger White Dwarf Binaries in the Galactic Bulge Time Domain Survey

Short-period Galactic white dwarf binaries detectable by LISA are the only guaranteed persistent sources for multi-messenger gravitational-wave astronomy. Large-scale surveys in the 2020s present an opportunity to conduct preparatory science campaigns to maximize the science yield from future multi-messenger targets. The Nancy Grace Roman Space Telescope Galactic Bulge Time Domain Survey will (in its Reference Survey design) image seven fields in the Galactic Bulge approximately 40,000 times each. Although the Reference Survey cadence is optimized for detecting exoplanets via microlensing, it is also capable of detecting short-period white dwarf binaries. In a recent paper entitled "LISA Galactic Binaries in the Roman Galactic Bulge Time-Domain Survey" (arXiv:2212.14887), we presented conservative forecasts for the number of detached short-period binaries the GBTDS will discover, and the implications for the design of electromagnetic surveys. Although population models are highly uncertain, we found a high probability that the baseline survey will detect of order ~5 detached white dwarf binaries. The Reference Survey would also have a >20% chance of detecting several known benchmark white dwarf binaries at the distance of the Galactic Bulge.<br><br>One consideration for optimizing the GBTDs for binary white dwarfs is ensuring that the visits to the individual fields are not precisely periodic to mitigate aliasing. A survey more specifically optimized for detecting binary white dwarfs would also include some continuous blocks of higher-cadence exposures of individual fields, rather than slewing between the fields for every exposure.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Binary stars / Trinary stars, White dwarf stars, Neutron stars, Stellar populations, Stellar evolution

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Rachel Street
Las Cumbres Observatory

Y. Tsapras, Heidelberg University; E. Bachelet, Caltech/IPAC; J. Sobeck, CFHT; P.M.McGehee, SLAC; M. Dall'Ora, INAF-OACN; M. Hundertmark, Heidelberg University;M.Di Criscienzo, INAF-OAR; M. Makler, ICAS-UNSAM & CBPF, M. Rabus, Universidad Católica de la Santísima Concepción, K. Dage, McGill University, W. Clarkson (University of Michigan-Dearborn); S. Khakpash, Rutgers University, Benjamin Montet, University of New South Wales, N. S. Abrams, UC Berkeley

Optimizing the science return from simultaneous NIR and Optical Timeseries photometry in the Galactic Bulge
Over the next decade, the overlap of two groundbreaking surveys offers us a chance to characterize time-variable phenomena in the Galactic Bulge to an unprecedented degree.<br><br>The Nancy Grace Roman Space Telescope will deliver exquisitely high precision NIR timeseries photometry and astrometry of millions of stars in the Galactic Bulge once it launches in ~2026. The Vera C. Rubin Observatory will provide contemporaneous timeseries photometry in optical passbands, after its commissioning in late 2024.<br><br>The combined data from these two great observatories will cover key passbands in the Spectral Energy Distributions of most stars, allowing us to measure the properties of stars in the Roman Galactic Exoplanet Survey (RGES). But complementary time-domain coverage of these objects will enable the characterization of a wide range of stellar variability, such as Cepheids and RR Lyrae that will help us to trace galactic structure to greater distances thanks to these survey's fainter limiting magnitudes. It can also help to measure the parameters of exoplanet transits detected by Roman, and to rule out blending by stellar binaries in these crowded regions.<br><br>By coordinating the survey strategies of both Roman and Rubin, we can enhance the scientific return of the RGES. Roman's coverage of the Galactic Bulge will necessarily suffer gaps of several months between survey periods. Rubin observations during these periods will help to constrain the morphology of microlensing lightcurves after Roman stops observations, which is particularly important for verifying the microlensing parallax, and could allow us to detect additional anomalous features. For this reason, we propose further exploration of the scientific benefits of inter-season gap coverage as well as near-simultaneous observations by Rubin of the RGES fields. By understanding what observations can be delivered within the constraints of both major surveys, the community will also be able to explore how co-survey observations from other ground-based facilities, such as the PRIME telescope and DECam on the Blanco 4m, can enhance the overall science return.

Galactic Bulge Time Domain Survey

exoplanets and exoplanet formation, stellar physics and stellar types, stellar populations and the interstellar medium, microlensing detection of exoplanets, survey strategy optimization, stellar variability

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Radek Poleski
Astronomical Observatory, University of Warsaw

Bulge Initial Mass Function

Our understanding of the mass function of low-mass stars is limited to the Solar neigbourhood. This limitation further restricts our knowledge of the Initial Mass Function (IMF) or dark matter content in the Galactic bulge. The low-mass stars are observed in the Galactic bulge (most importantly by the Hubble Space Telescope) but we cannot translate observed luminosity function into a mass function because we do not have proper statistics of stellar binary systems. The low-mass stellar binaries located a few kpc away cannot be spatially resolved, nor can they be found using radial velocity shifts. The Roman Galactic Exoplanet Survey (RGES) has potential to significantly increase our understanding of binarity statistics in the disk and in the bulge, which then can be used to calculate the IMF as a function of galactocentric distance or the dark matter content in the Galactic bulge. First, the RGES will provide catalogs of stars that will include even the lowest-mass stars in the bulge. Second and more importantly, the RGES will provide thousands of microlensing events with stellar binaries as either lenses or sources. For each of these events we will be able to measure projected separations and either a mass ratio (binary lens events) or a flux ratio (binary source events). Thanks to higher-order microlensing effects (microlensing parallax, finite source effect, astrometric shift, or detection of the lens flux), we will measure distances to the lenses. All these quantitites allow constraining the binarity statistics with accuracy not possible currently with ground-based microlensing searches and the Hubble Space Telescope luminosity function.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, stellar populations and the interstellar medium, Binary stars / Trinary stars, Low mass stars, Gravitational microlensing, Galaxy bulges, Galaxy disks

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Susmita Das
Konkoly Observatory, CSFK, Budapest

László Molnár

Discovering new BLAPs in the Galactic plane

Blue large-amplitude pulsators (BLAPs) represent a new class of extremely rare and hot pulsating stars with unusually large amplitudes and short periods (in the range of 20-40 min). These stars exhibit sawtooth light curves, similar to those of RR Lyraes and classical Cepheids. The evolutionary status of these stars remains unknown; however, pulsation theory predicts that they may be evolved low-mass stars with inflated helium-enriched envelopes.<br><br>Ever since the discovery of the first 14 BLAPs from the OGLE-IV survey, these rare stars have also been discovered by other surveys like Gaia DR2 and ZTF DR3. Their rare occurrence is thought to be because of their evolutionary history within interacting binary systems and their short timescales over which they transition the instability strip. All the BLAPs currently known are located in the Galactic plane with magnitudes in the range 15-19 mag. In addition to being rare, certain observational limitations may hinder their detection. BLAPs have intrinsically blue colors and the interstellar dust in the Galactic plane may prevent these sources from being easily identified. Roman could thus prove instrumental in discovering many additional new BLAPs and in unlocking their origin with its high sensitivity, high cadence and precise photometry, especially within the Galactic plane.

Galactic Bulge Time Domain Survey

stellar physics and stellar types, Variable stars, Stellar evolution

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Thomas Barclay
UMBC

Robert F. Wilson

Stellar characterization in the Galactic Bulge Fields

Roman observations of the Galactic Bulge provide unprecedented access to this region of the Galaxy. In addition to enabling exoplanet microlensing, these data will support numerous science investigations including the study of transiting exoplanet, asteroseismology, stellar flares, and eclipsing binaries. However, these investigations all rely to varying degrees on being able to determine the properties of the stars in the bulge fields. With 10's of millions of stars, and high stellar density, this is not a trivial problem as the bulge fields are not amenable to Gaia observations. Fortunately, the Roman Wide Field Instrument provides the capabilities to greatly enhance stellar characterization through the use of the the filters. By collecting images using all 8 Roman filters we could determine accurate stellar properties of all the stars in the bulge fields. These images need not be collected regularly; a few times per observing season would be sufficient. A minimal investment in observing resources would provide a large enhancement in science return.

Galactic Bulge Time Domain Survey

exoplanets and exoplanet formation, stellar physics and stellar types, stellar populations and the interstellar medium, Planet hosting stars, Exoplanets, Binary stars / Trinary stars, Stellar distance, Evolved stars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Peter Nugent
LBNL / UC Berkeley

Nao Suzuki

Enhanced Transient Science with Roman + LS4

The The La Silla Schmidt Southern Survey (LS4) is a 5 year public, wide-field, optical survey using an upgraded 20 square degree QUEST Camera on the ESO Schmidt Telescope. LS4 will have first light at the end of 2023 and the survey will commence in early 2024. We will use LBNL fully-depleted CCDs to maximize the sensitivity in the optical up to 1 micron. This survey will complement the Legacy Survey of Space and Time (LSST) being conducted at the Vera C. Rubin Observatory in two ways. First, it will provide a higher cadence than the LSST over several thousand square degrees of sky each night, allowing a more accurate characterization of brighter and faster evolving transients to 21st magnitude. Second, it will open up a new phase-space for discovery when coupled with the LSST by probing the sky between 12-16th magnitude - a region where the Rubin Observatory saturates. The science goals of LS4 include obtaining a large sample of nearby supernovae to probe both supernova physics and cosmology including peculiar velocities; follow up of multi-messenger astrophysical transients including gravitational wave events, GRBs, and neutrinos; tidal disruption events; AGN and quasar variability studies; stellar physics in the Milky Way; and other unexpected short duration transients. Through coordination with Roman, and joint analysis of the data, we would be able to extend the science reach of both projects considerably in a similar way to what we have proposed doing with the LSST on Rubin - here extending the science impact to the near infrared.

High Latitude Time Domain Survey

stellar physics and stellar types, galaxies, supermassive black holes and active galaxies, large scale structure of the universe, supernova, Variable stars, AGB, GRB, Cosmological parameters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Sam Grunblatt
Johns Hopkins University

Measuring Distances to The Edge of Our Galaxy and Beyond With TRGB Star Oscillations

Stars near the tip of the red giant branch of stellar evolution oscillate with frequencies which are directly correlated with their luminosity and surface gravity. These pulsations have timescales of days to weeks, and thus can be observed in a survey with 5-day cadence over a 2 year baseline. As these stars are so intrinsically bright, observations in a filter between 1 and 2 microns that achieve 10 parts per thousand precision of a 18th magnitude star in H-band can be used to measure the oscillations and thus distances of stars hundreds of kiloparsecs away. These distances can then be used to determine the effective stellar 'edge' of the Milky Way, beyond which no more halo stars are found, important for understanding the formation of our Galaxy and the role of dark matter in shaping its potential. Furthermore, these observations can provide precise distances to nearby galaxies, and will also allow measurement of the distances to stars associated with the Andromeda Galaxy. These observations can be use as benchmarks for determining the potential of the Local Group with implications for galactic dynamics at several Mpc distances.

High Latitude Time Domain Survey

stellar populations and the interstellar medium, evolved stars, stellar distances, galaxy halos
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Yuichi Harikane
University of Tokyo

M. Oguri (Subaru Advisory Committee, Chair), T. Kodama, M. Ouchi, A. Nishizawa, H. Miyatake, Tsutomu T. Takeuchi, K Nakajima, Tomomi Sunayama、Masayuki Tanaka, A. K. Inoue

Maximizing the Synergy between Roman and Subaru

The combination of joint Roman and Subaru observations has the potential to enable transformative science that cannot be done by either telescope alone. The wide field of views of Subaru/Hyper Suprime-Cam (HSC, 1.5 deg2) and Prime Focus Spectrograph (PFS, 1.2 deg2) have excellent synergies with Roman's wide field instruments. Roman will image the 0.6-2.1um sky with unprecedented depth and area, and Subaru/HSC will provide broad-band and unique narrow- and medium-band images at 0.4-1.0 um complementary to Roman. The Subaru/PFS will conduct massive spectroscopic observations (~2400 fibers/pointing) with the medium resolution (R~3000) at 0.38-1.26um, which will complement Roman's grism spectroscopy at 1.0-1.9um with R~300. The director of the Subaru Telescope and Subaru Advisory Committee already agreed with NASA to commit 100 Subaru nights to the Roman-Subaru synergetic observations.<br><br>To enable the Roman and Subaru synergetic observations, we propose to observe northern and equatorial fields that can be observed with Subaru. The possible field candidates include Chandra Deep Field South, North Ecliptic Pole, and COSMOS, all of which are accessible from Subaru and with low Galactic extinction. By taking advantage of the unique capabilities of Subaru/HSC and PFS, the Roman and Subaru/HSC+PFS synergetic observations will allow us to investigate various important science cases to understand galaxy formation and evolution, such as discoveries of luminous early galaxies at z>10 (with deep non-detection bands from Subaru to eliminate interlopers) currently showing a tension with theoretical predictions, large scale structures and protoclusters at z=2-15, mapping the progression of cosmic reionization with improved redshift precision of galaxies enabled with HSC/narrow-bands+Roman, the most massive galaxies to study their possible tension with the LCDM cosmology up to z~4, and metal-poor star-forming galaxies in the early evolutionary phase at z=1-2 possibly hosting primordial structures such as Pop-III stars, all of which can be only identified in the wide-area Roman and Subaru synergetic observations. Furthermore, the medium-band images from Subaru/HSC will greatly improve the accuracy of the photometric redshift which is crucial for weak lensing cosmology. Thus, choosing fields that can be accessible from Subaru as the core community survey field will maximize the scientific outputs from Roman and Subaru synergetic observations.

High Latitude Time Domain Survey


galaxies, the intergalactic medium and the circumgalactic medium, supermassive black holes and active galaxies, large scale structure of the universe, Galaxy evolution, Galaxy formation, Cosmology, Large-scale structure of the universe, Reionization

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Aaron Meisner
NSF's NOIRLab

A New Window into the Milky Way's Structure and History

Modern optical surveys have enabled tomography of the Milky Way using populations such as main sequence turnoff stars. The Milky Way's cold, substellar population also carries a wealth of information about our Galaxy's structure and the star formation process at low masses, but thus far studies of these coolest objects have been limited to the Sun's very local neighborhood. The combination of deep near-infrared and red-optical survey data from Roman and Rubin will vastly expand the volume covered by samples of cold (sub)stellar objects, allowing us to: map the Galaxy's scale height into the L and T spectral classes, understand any metallicity dependence toward the bottom of the substellar mass function, characterize the stellar/substellar boundary's evolution with metallicity, trace low-mass star formation over cosmic time, and probe the age versus temperature relation of brown dwarf cooling.<br><br>Sample selection will be a primary challenge in this endeavor. Rubin naturally complements Roman in identifying distant substellar objects, through the extended wavelength coverage it affords into the optical and the lengthened Roman+Rubin time baseline available for proper motions. Tools for joint analysis of Roman+Rubin survey data archives would help enable this science case, particularly cross-matched catalogs, homogenized astrometry, and ideally "forced photometry" of each survey's detections in the other's imaging. It is important for this science application that the Roman High Latitude Wide Area Survey include imaging in Roman WFI's K-band equivalent filter (F213), as this bandpass is critical for photometric selection of brown dwarfs, particularly distant ultracool dwarfs in the Milky Way's thick disk and halo (see e.g., Figure 1 of Stauffer et al. 2019, BAAS, 51, 94).

High Latitude Wide Area Survey


stellar physics and stellar types, brown dwarfs, infrared photometry, low mass stars, late-type stars, astrometry

Akio Inoue
Waseda University

GREX-PLUS mission team

Enhancing the value of Roman Core Community Surveys with GREX-PLUS wide-area imaging surveys in wavelengths longer than two micron

The Roman Space Telescope will conduct unprecedented wide-area surveys in near-infrared wavelengths up to 2 micron. However, there are many important science cases achievable if the Roman survey is supplemented by similarly wide-area surveys in wavelengths longer than 2 micron. An extension of the spectral coverage of objects detected in the Roman surveys to better understand their spectral energy distribution is the simplest benefit. There should also be many populations not detected in Roman images but detected in wavelengths longer than 2 micron, such as extremely low temperature stars, dust-obscured stars, dusty high redshift galaxies and active galactic nuclei, and even star-forming galaxies at extremely high redshifts beyond redshift of 15. While the James Webb Space Telescope has the extremely high sensitivity in the wavelength range, it may not achieve any survey with a more than square degree area due to the narrow field-of-view. A Japanese future space telescope mission candidate, GREX-PLUS (Galaxy Reionization EXplorer and PLanetary Universe Spectrometer) plans to have a wide-field camera in a wavelength range of 2 to 8 micron and aims to conduct ~10--1,000 square degree wide-area imaging surveys. The imaging depths are ~27--24 AB magnitude depending on the survey area and the wavelength band. Although these depths are somewhat shallower than those of the Roman surveys, the wide-area survey ability of GREX-PLUS in wavelengths longer than 2 micron is only the solution to supplement the longer wavelength coverage to the Roman surveys limited to 2 micron. The target launch year of GREX-PLUS is early 2030s.<br><br>To maximize the synergy of the two wide-field imaging surveyors, Roman and GREX-PLUS, both telescopes should observe the same areas. Since GREX-PLUS will also orbit around the Sun-Earth L2 point, as will Roman, the sky area visibility will be the same. Therefore, GREX-PLUS will observe the sky areas where Roman observed in its Core Community Surveys and in General Observer programs for extragalactic fields and for the Galactic plane as well. Since there is a partial spectral overlap between Roman's F213 filter and GREX-PLUS's F232 filter, it would be highly beneficial to coordinate the Roman F213 imaging observations with the GREX-PLUS surveys in respect to the depth and area.

High Latitude Wide Area Survey

solar system astronomy, exoplanets and exoplanet formation, stellar physics and stellar types, stellar populations and the interstellar medium, galaxies, the intergalactic medium and the circumgalactic medium, supermassive black holes and active galaxies, large scale structure of the universe

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

John Bally
Astrophysical and Planetary Sciences, University of Colorado, Boulder

Jets, Outflows, and Shocks in from Forming & Dying Stars in The Milky Way

I propose a survey of the Galactic Plane and some nearby off-plane star-forming molecular clouds with Roman. A survey of the fields covered by the Spitzer near-IR (GLIMPSE), mid-IR (MIPSGAL), and Herschel far-IR (Hi-GAL) surveys with Roman's ~0.1 arc-second resolution will provide a wealth of information on Galactic stellar populations, star-formation, stellar death, the interstellar medium (ISM), and the feedback processes that regulate the ISM's state. A re-observation in a decade after the first survey will measure Galactic stellar proper motions<br><br>Most astrophysical systems which rotate, accrete, and have magnetic fields power jets and bipolar outflows. Examples include protostars, dying stars, symbiotic binary systems, neutron stars, and black holes surrounded by accretion disks. Accretion-powered jets and outflows share many similarities despite orders of magnitude differences in mass and size scales. Their morphologies tend to be similar: highly collimated, bipolar beams near the source which break into chains of bow shocks farther out. Outflow speeds tend to be a few times the equivalent circular orbit speed where the outflow is launched - a few hundred km/s for protostars and near the speed of light for black holes and neutron stars.<br><br>Most young stellar objects (YSOs) and many post-main-sequence stars drive jets and bipolar outflows while they accrete. These objects constitute the nearest class of accretion-powered jets and outflows. Due to their proximity, structural changes and proper motions can be measured on time-scales ranging from weeks to decades. Studies of these systems provide nearby laboratories for the investigation of all classes of accretion powered outflow systems.<br><br>Roman's broad-band filters can identify extended nebulosity produced by shocks, ionized nebulae powered by young massive stars, supernova remnants and stellar wind bubbles, enable powered by recently collapsed stellar cores (planetary nebulae). Specifically, the emission lines of hydrogen (1.87 um Paschen-alpha, etc.) trace visually obscured ionized nebulae and recombining plasma behind shocks. Shocks are particularly bright in the 1.644 um line of [FeII] when propagating into atomic media, and the 2.12 um line of molecular hydrogen when propagating into molecular media. These extended nebulosities can be identified by morphology and distinguished from scattered or continuum emission (e.g, from unresolved stars) by image arithmetic. For example, the 1.87 um HI and 2.12 um molecular hydrogen line emission regions can be identified by differencing the F184 and F213 filter images. This works because the two emission lines trace very different environments and are usually spatially separated.<br><br>Visual to near-infrared, wide-field surveys with Roman of the Galactic Plane and nearby low-Galactic-latitude star-forming clouds such as Taurus, Orion, and Perseus can be used to identify outflows from forming and dying stars.<br><br>The goals of Galactic plane surveys are:<br><br>- Identify large populations of young stellar objects, protostellar outflows, HII regions, stellar wind-bubbles, proto-planetary and planetary nebulae.<br><br>- Observe the Hi-Gal and Spitzer fields with sub-arcsecond resolution in all Roman filters: The Galactic plane plus off-plane clouds require about 1,000 square degrees. 360 x 2 degrees along the Galactic plane, and about 280 square degree off the plane which contains star-forming clouds such as Orion , Taurus, and Perseus.<br><br>- Special emphasis will be to study the Central Molecular Zone of the Milky Way which comprises the central ~500 pc of the Galaxy, and serves as a nearby analog of star-birth in high-pressure environments thought to occur in the high-redshift Universe.<br><br>- A repeat of the survey in the near-IR filters about a decade after the initial observations will reveal Galactic stellar proper motions not observable with Gaia.<br><br>Roman Galactic surveys provide the "ground-truth" for interpreting the physics of star-formation, stellar death, and feedback which regulates the physical and chemical states of galactic interstellar media.<br><br>Note: Narrow-band filters tuned to the 1.64 um, 1.87 um, and 2.12 um emission lines would be extremely useful additions to Roman's complement of broad-band filters. These filters would enable observations of brighter stars, and would improve Roman's ability to study the ISM. These filters wold also be useful for identification of high-redshift emission-line galaxies at specific redshifts.

High Latitude Wide Area Survey

stellar physics and stellar types, stellar populations and the interstellar medium, astrometry, HII regions, interstellar medium, stellar jets, protostars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Kathleen Kraemer
Boston College

Martha Boyer (STScI) Steve Goldman (STScI) Caroline Huang (Harvard-Smithsonian CfA) Atefeh Javadi (IPM) Abby Lee (Univ. Chicago) Noriyuki Matsunaga (Univ. Tokyo) Iain McDonald (Univ. Manchester) Nami Mowlavi (Univ. Geneva) Peter Scicluna (ESO) Greg Sloan (STScI) Sundar Srinivasan (UNAM) Michelle Trabucchi (Univ. Geneva) Alfonso Trejo (UNAM) Jacco van Loon (Keele Univ.) Diego Alejandro Vasquez (UNAM) Patricia Whitelock (SAAO)

Setting the Stage for Improving the Distance Ladder with Roman Core Community Surveys

Background: The upcoming Nancy Grace Roman mission offers an unprecedented opportunity to improve the cosmic distance ladder, and the Core Community Surveys (CCS), if properly designed, can play a key role in this endeavor. The use of long period variable stars (LPVs) as standard candles can extend our reach beyond the limits achievable with Cepheids, since the intrinsic luminosities of the LPVs are significantly higher and hence can be detected at larger distances. Recent work has calibrated the "J-AGB" method using J-band photometry and Gaia distances for Galactic carbon stars (Lee et al. 2021, 2022), and Hubble near-IR photometry of oxygen-rich Miras in supernova host galaxies (Huang, Riess, et al. 2018, 2020). A significant limit of the method to date, though, is the small number of galaxies to which it has been applied, largely due to limits of current facilities (fields-of-view, no/limited near-IR bands, sensitivity, insufficient revisit rate, etc.).<br><br>Proposed science investigation: All three of the planned Core Community Surveys have the potential to impact this field. The most important will be the High Latitude Wide Area Survey with its large area, 2-year survey using the Y106, J129, H158, F184 filters + Grism. In terms of this call for science concepts and the CCS design, the key is to maximize the number of galaxies in the survey regions for which LPVs can be detected. These multi-band data will enable us to identify and characterize the evolved star populations in these galaxies. Thus, as the survey is designed in detail, the exact locations of the pointing centers should be optimized to include these galaxies. As most of the science cases will be using data from well within the survey footprint, a small pointing adjustment to include more of our target galaxies should be transparent to other users in the community but could improve our studies significantly.

High Latitude Wide Area Survey


stellar physics and stellar types, stellar populations and the interstellar medium, galaxies, evolved stars, stellar distance, variable stars, infrared photometry, stellar populations

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Keith Bechtol
University of Wisconsin-Madison

Peter Ferguson, Nushkia Chamba, Alex Drlica-Wagner, Jeffrey L. Carlin, Ethan O. Nadler, Andrew Pace, Burcin Mutlu-Pakdil, Nora Shipp, Will Clarkson, Annika Peter, Jennifer Sobeck, Kristen Dage

Coordinating Roman and Rubin Surveys for Cosmic Probes of Dark Matter

We are interested in coordination between the Nancy Grace Roman Space Telescope and the Vera C. Rubin Observatory to enhance cosmic probes of dark matter. Astrophysical observations probe the physics of dark matter through its impact on structure formation throughout cosmic history. Fundamental properties of dark matter - e.g., particle mass, self-interaction cross section, coupling to the Standard Model, and time evolution - can imprint themselves on the macroscopic distribution of dark matter in a detectable manner by modifying the abundance, density profiles, and spatial distribution of dark matter halos. Astrophysical observations offer unique sensitivity to a wide range of dark matter particle models (including particle candidates that interact only through gravity) and are highly complementary to terrestrial experiments and indirect dark matter searches. Additionally, measurements of the dark matter distribution across a wide range of physical length scales can be used to constrain the physics of the early Universe, including inflation as well as non-standard cosmologies, e.g., with early matter domination.<br><br>In the coming years, Roman-Rubin coordination could enhance studies of dark matter halos that are below the minimum mass threshold to host stellar populations. This halo mass range below 10^8 solar masses is the next observational frontier. These halos offer unique advantages to constrain the microphysical properties of dark matter because their evolution is less affected by complicated baryonic physics and because many "non-minimal" dark matter properties leave the most conspicuous signatures on low-mass halos. We highlight two example opportunities for Roman-Rubin coordination.<br><br>(1) The combination of optical (Rubin) + space-based near-IR (Roman) imaging would allow efficient star-galaxy separation to enable detailed studies of the Milky Way stellar halo and ultra-faint galaxies several Mpc beyond the Milky Way virial radius (taking full advantage of unprecedented depth of both surveys). We would be able to conduct a detailed census of the low-mass galaxies throughout the Local Volume to firmly establish the threshold halo mass for galaxy formation (likely around 10^8 solar masses), and search for density perturbations in stellar streams caused by interactions with even lower-mass dark matter halos (10^6 - 10^8 solar masses).<br><br>(2) We could use the combination of Roman-Rubin to identify thousands of galaxy-scale strong lenses (taking advantage of optical to near-IR colors), and utilize the space-based angular resolution of Roman to select optimal candidates for follow-up observations with other facilities. There are two ways to use strong lensing to study low-mass dark matter halos within the main deflector and along the line of sight: flux-ratio anomalies and gravitational imaging (distortion of arcs). In combination with dedicated follow-up observations (e.g., JWST, ELTs), we would aim to access properties of dark matter halos in the mass range 10^6 to 10^7 solar masses.<br><br>Both of the techniques above benefit from large sky areas covered with both Roman and Rubin. It would be optimal to have a wide-area survey with Roman covering the majority of the LSST footprint in at least one band. This approach would combine multiband deep optical photometry from LSST with space-based resolution from Roman. For the star-galaxy separation use case, joint pixel processing, or at least forced photometry, would be important to ensure consistent object detection and photometry between the two datasets, and we need robust color measurements to take full advantage of the separation of galaxy and stellar loci in optical + near-IR color space. We note that similar survey concepts have been considered for other cosmology science cases, e.g., for weak gravitational lensing and galaxy clustering probes of dark energy https://arxiv.org/abs/2004.04702.

High Latitude Wide Area Survey

stellar populations and the interstellar medium, galaxies, large scale structure of the universe, Galaxies:Galaxy dark matter halos, Galaxies:Dwarf galaxies, Large Scale Structure of the Universe:Dark matter distribution, Large Scale Structure of the Universe:Gravitational lensing, Stellar Populations (and the ISM):Dwarf galaxies

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
Kristen Dage
McGill University

Christopher Usher, (Stockholm University, Sweden); Jennifer Sobeck, (CFHT, USA); Ana Chies Santos (UFRGS, Brazil); Robert Szabo (Konkoly Observatory, Hungary); Marta Reina-Campos (McMaster University, Canada); Léo Girardi (INAF-Padova, Italy); Vincenzo Ripepi (INAF-Capodimonte, Italy); Marcella Di Criscienzo (INAF-Rome, Italy); Ata Sarajedini (Florida Atlantic University, USA); Will Clarkson (University of Michigan-Dearborn, USA); Peregrine McGehee (SLAC, USA), Katherine Rhode (Indiana University, USA)

Extragalactic Star Cluster Science with the Nancy Grace Roman Space Telescope and the Vera C. Rubin Observatory

Star clusters provide a window onto a wide range of astrophysical processes and hold the answers to key questions regarding how stars form, evolve, and die, as well as how galaxies form and evolve. Moreover, observational and theoretical studies have demonstrated that globular clusters are effective probes of the shape and structure of their host galaxies, including the galaxies' dark matter halos. Synergistic observations from the Nancy Grace Roman Space Telescope's High Latitude Wide Area Survey and the Vera C. Rubin Observatory's Legacy Survey of Space and Time will allow for an entirely new characterization of extragalactic star clusters, reaching the turnover of the cluster luminosity function at distances out to 100 Mpc. Combining data from the two surveys will enable us to analyze stellar populations across the broadest wavelength range yet achieved, and Roman's higher spatial resolution will allow us to estimate the sizes of globular clusters in external galaxies with a wide range of properties and environments. Measurements in blue optical filters from Rubin are crucial for globular cluster science, because near-infrared photometry alone is not sufficient to break the age-metallicity and age-extinction degeneracies. The latter is a fundamental issue in studies of stellar populations in star-forming galaxies.<br><br>The core synergies between the two facilities will drastically improve our understanding of stellar populations and host galaxy assembly, but will also help us understand the populations of exotic stellar objects found within globular clusters (and by extension, the progenitor sources of gravitational wave events). Observing extragalactic globular clusters with Roman alone will allow us to measure globular cluster metallicities, but breaking the age/metallicity degeneracy requires data from both Rubin and Roman. Breaking this well-known degeneracy will make us more effective at selecting and studying extragalactic star clusters and will represent a major step forward in our understanding of the assembly history of galaxies and their dark matter content. Roman's excellent spatial resolution will provide information on the sizes and structures of the globular clusters; this information, when paired with age/metallicity measurements, can be combined with multiwavelength observations to securely link globular cluster properties to stellar exotica, including the progenitors of merging black hole black-hole binaries.

High Latitude Wide Area Survey

stellar physics and stellar types, stellar populations and the interstellar medium, galaxies, globular clusters, stellar populations, black holes, X-ray binaries

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Matthew De Furio
University of Michigan - Ann Arbor

Michael R. Meyer

Pushing the Limits of Star Formation Theory: An in Depth Exploration of Large Star-forming Regions

Star forming regions contain clues to uncovering the details of the star formation process. They have a wide variety of environmental properties, ranging from very low density associations with few stars to very high density, bound clusters with hundreds of thousands of stars. Past studies have identified no difference between the distribution of masses, the initial mass function (IMF), within various stellar populations, although this remains unclear for sub-stellar objects down to the limit of turbulent fragmentation, ~ Jupiter mass scales (Bastian et al. 2010). Importantly, environmental differences have been identified within the stellar multiple populations of Taurus (a low-density association) and the Orion Nebula Cluster (a high-density cluster), likely due to dynamical encounters during states of very high density (De Furio et al. 2022). With the Nancy Grace Roman Space Telescope (Roman), we can probe star formation properties within a wide variety or star-forming environments in order to: a) define the stellar and sub-stellar membership unattainable from the ground or other space-based telescopes, b) define the limit of turbulent fragmentation, the very low mass end of the IMF, and identify any potential environmental impacts (e.g. metallicity, presence of OB stars), and c) characterize the multiple populations down to planetary mass primaries and angular resolutions of ~ 100 milli-arcseconds (mas).<br><br>Current work with the James Webb Space Telescope (JWST) is designed to explore the very low mass end of the IMF in dense embedded clusters. While no other telescope can match the sensitivity of JWST in the infrared, the field of view of NIRCam is nearly 100x smaller than that of the wide-field instrument on Roman. On the other hand, ground-based telescopes are not sensitive enough to the low-mass sub-stellar population, particularly when extincted, and cannot attain high angular resolution over a large field of view. Space-based survey telescopes (like Gaia) are also not sensitive to the faint sub-stellar members of star-forming regions and suffer from extinction in the visible. Roman is crucial to observing regions on large angular scales like OB associations, those with thousands of stars and potentially the most common location of star formation, in order to explore the fundamental features of the star formation process. Roman is the only observatory that can be used to characterize the sub-stellar content across large scale star-forming regions in the near infrared and have the efficiency to explore multiplicity down to separations of 100 mas across entire star-forming regions. With the observations of dozens of star-forming regions, across 0.5-2.3µm, Roman will serve as the gold-standard in star formation astrophysics, complementary to work done by JWST in deeply embedded clusters, and provide a large database for future archival research in areas like the formation and evolution of protoplanetary disks.

High Latitude Wide Area Survey


stellar physics and stellar types, stellar populations and the interstellar medium, Star formation, Star clusters, Brown dwarf stars, Binary stars / Trinary stars, Pre-main sequence stars

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Robert Blum
Rubin Observatory/NSF's NOIRLab

Federica Bianco (Rubin Observatory/U Delaware), Leanne Guy (Rubin Observatory), Zeljko Ivezic (U Washington/Rubin Observatory, Steve Ritz (UC Santa Cruz/Rubin Observatory), Tony Tyson (UC Davis/Rubin Observatory)

Rubin proposal for a single-band Roman survey covering the LSST Wide-Fast-Deep footprint

In early 2025, the Vera C. Rubin Observatory will begin executing the Legacy Survey of Space and Time (LSST, Ivezić et al., 2019 ApJ, 873, 111). The bulk of the 10-year LSST program will be dedicated to the Wide-Fast-Deep (WFD) survey, which will cover the sky to unprecedented depths in the u,g,r,i,z,y photometric bands over an area from the south celestial pole up to a declination of ~ +15 degrees. Roman and Rubin are highly complementary in wavelength, angular resolution, and time domain coverage. This proposal presents the case for a single-band Roman community survey with LSST-matched depth over the LSST WFD footprint to enhance the key science programs of both missions. The almost one order of magnitude enhanced angular resolution of Roman will boost deblending of faint galaxies and crowded regions in the Galactic plane leading to valuable and enhanced scientific impact over many of Rubin's and Roman's science goals; and would also lead to improved Differential Chromatic Refraction (DCR) modeling. Roman's extended wavelength range provides several key enhancements: improved estimates of photo-z for galaxies at all redshifts and hence improved cosmological parameter estimation; extended redshift limit for a given photo-z accuracy, thus extending the range of cosmic time for studying galaxy evolution; and improved simultaneous estimates of stellar distances and the dust column along the line of sight in the Galactic plane. Time domain data from LSST compliments Roman; flickering and variable compact objects within galaxies may be studied in new ways.<br><br>Assuming 100 sec Roman exposures with 65% efficiency (due to slew and settle), we estimate that about four months, not necessarily contiguous, are required to cover the LSST WFD footprint to mAB = 25.5 in a single band (about 1.5 mag deeper than Euclid survey). The optimal single Roman band will require quantitative optimization over several of the leading science cases outlined above.

High Latitude Wide Area Survey

solar system astronomy, exoplanets and exoplanet formation, stellar physics and stellar types, stellar populations and the interstellar medium, galaxies, the intergalactic medium and the circumgalactic medium, supermassive black holes and active galaxies, large scale structure of the universe, Cosmological parameters, Dark matter distribution, Near-Earth objects, Galaxy evolution, Supernovae

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Ting Li
University of Toronto

Exploring Milky Way's stellar streams, dwarf galaxies and star clusters with Roman

Roman will be powerful tool to explore the substructure and satellite systems in the Milky Way. With its high precision photometry to high depth, well-calibrated astrometric measurements on proper motion, we will be able to use them to study the formation history of the Milky Way as well as shed light on the nature of dark matter. It will be very useful if the footprint and survey strategy for the Roman high-latitute survey would be carefully designed to coordinate with the planned or existing surveys such as the LSST on Rubin Observatory, and DESI survey at KPNO, etc., to maximize its scientific potential.

High Latitude Wide Area Survey

stellar populations and the interstellar medium, galaxies, Galaxy dark matter halos, Dwarf galaxies, Galaxy halos, Globular star clusters, Star clusters

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Yuichi Harikane
University of Tokyo

M. Oguri (Subaru Advisory Committee, Chair), T. Kodama, M. Ouchi, A. Nishizawa, H. Miyatake, Tsutomu T. Takeuchi, K Nakajima, Tomomi Sunayama、Masayuki Tanaka, A. K. Inoue

Maximizing the Synergy between Roman and Subaru

The combination of joint Roman and Subaru observations has the potential to enable transformative science that cannot be done by either telescope alone. The wide field of views of Subaru/Hyper Suprime-Cam (HSC, 1.5 deg2) and Prime Focus Spectrograph (PFS, 1.2 deg2) have excellent synergies with Roman's wide field instruments. Roman will image the 0.6-2.1um sky with unprecedented depth and area, and Subaru/HSC will provide broad-band and unique narrow- and medium-band images at 0.4-1.0 um complementary to Roman. The Subaru/PFS will conduct massive spectroscopic observations (~2400 fibers/pointing) with the medium resolution (R~3000) at 0.38-1.26um, which will complement Roman's grism spectroscopy at 1.0-1.9um with R~300. The director of the Subaru Telescope and Subaru Advisory Committee already agreed with NASA to commit 100 Subaru nights to the Roman-Subaru synergetic observations.<br><br>To enable the Roman and Subaru synergetic observations, we propose to observe northern and equatorial fields that can be observed with Subaru. The possible field candidates include Chandra Deep Field South, North Ecliptic Pole, and COSMOS, all of which are accessible from Subaru and with low Galactic extinction. By taking advantage of the unique capabilities of Subaru/HSC and PFS, the Roman and Subaru/HSC+PFS synergetic observations will allow us to investigate various important science cases to understand galaxy formation and evolution, such as discoveries of luminous early galaxies at z>10 (with deep non-detection bands from Subaru to eliminate interlopers) currently showing a tension with theoretical predictions, large scale structures and protoclusters at z=2-15, mapping the progression of cosmic reionization with improved redshift precision of galaxies enabled with HSC/narrow-bands+Roman, the most massive galaxies to study their possible tension with the LCDM cosmology up to z~4, and metal-poor star-forming galaxies in the early evolutionary phase at z=1-2 possibly hosting primordial structures such as Pop-III stars, all of which can be only identified in the wide-area Roman and Subaru synergetic observations. Furthermore, the medium-band images from Subaru/HSC will greatly improve the accuracy of the photometric redshift which is crucial for weak lensing cosmology. Thus, choosing fields that can be accessible from Subaru as the core community survey field will maximize the scientific outputs from Roman and Subaru synergetic observations.

High Latitude Wide Area Survey

galaxies, the intergalactic medium and the circumgalactic medium, supermassive black holes and active galaxies, large scale structure of the universe, Galaxy evolution, Galaxy formation, Cosmology, Large-scale structure of the universe, Reionization

